User Satisfaction in Competitive Sponsored Search

We present a model of competition between web search algorithms, and study the impact of such competition on user welfare. In our model, search providers compete for customers by strategically selecting which search results to display in response to user queries. Customers, in turn, have private preferences over search results and will tend to use search engines that are more likely to display pages satisfying their demands. Our main question is whether competition between search engines increases the overall welfare of the users (i.e., the likelihood that a user finds a page of interest). When search engines derive utility only from customers to whom they show relevant results, we show that they differentiate their results, and every equilibrium of the resulting game achieves at least half of the welfare that could be obtained by a social planner. This bound also applies whenever the likelihood of selecting a given engine is a convex function of the probability that a user's demand will be satisfied, which includes natural Markovian models of user behavior. On the other hand, when search engines derive utility from all customers (independent of search result relevance) and the customer demand functions are not convex, there are instances in which the (unique) equilibrium involves no differentiation between engines and a high degree of randomness in search results. This can degrade social welfare by a factor of the square root of N relative to the social optimum, where N is the number of webpages. These bad equilibria persist even when search engines can extract only small (but non-zero) expected revenue from dissatisfied users, and much higher revenue from satisfied ones.

==> se-pure-equil.tex <==
\section{When Satisfaction is Necessary: $\DF = 0$} 
\label{sec:beta0}

In this section, we analyze equilibria of the \SearchGameName
\SearchGame{0}{\TypeDist} when $\DF = 0$.
In this case, the utility of an engine is the total fraction of agents
that she attracts \emph{and satisfies}.
\bldelete{, leading to a better alignment
of engine payoff and searcher welfare.}
We will show that, for any type distribution in general position,
under a natural (and extremely weak) condition on
the selection rule \SelRule, all equilibria of the
\SearchGameName are deterministic. 
We use this result to compare the \SearchGameName
to a game in which engines are restricted to using
deterministic strategies. 
We show that this related game is a Valid Utility Game, and
infer that its Price of Anarchy is at most $2$; this implies the
same bound on the Price of Anarchy of the \SearchGameName.

\subsection{Deterministic Equilibria}
\label{sec:deterministic-equilibria}
We begin by defining a non-indifference property of selection rules.
Roughly speaking, we wish to exclude selection rules for which a
search engine's probability of satisfying a user has effectively no
impact on that user's selection.
We define the \emph{support} $S(\SatProbs)$ of a satisfaction
probability vector $\SatProbs$ to be the set of engines for which
$\SatProb{i} > 0$.   
We say that $\SelRule$ is \emph{non-indifferent} if, 
whenever $\SetCard{S(\SatProbs)} \geq 2$ 
and $\SatProb{j} < 1$ for some $j \in S(\SatProbs)$, 
there exists some $i \in S(\SatProbs)$ such that
$\SelRule[i](\SatProbs) < \SelRule[i](1, \SatProbs_{-1})$.
That is, if at least two engines would satisfy a user with positive
probability, and not all supporting engines satisfy the user with
probability $1$, then at least one supporting engine would be more
likely to attract the user by sufficiently increasing her probability
of satisfying him. 

The non-indifference property is quite weak; in particular, it is
significantly weaker than assuming that $\SelRule[i]$ is strictly
increasing in $\SatProb{i}$.
For example, both the Majority and Markovian selection rules described
in Section~\ref{sec:selection-rules} are not strictly increasing in the
satisfaction probabilities, but do satisfy non-indifference. 

%\paragraph{Aside: degeneracy of $\Gamma$}
%Given that $\beta = 0$ and $f$ is non-indifferent, we wish to show that all equilibria of the resulting game are pure.  However, this is not technically true: there are cases in which an engine might mix between choosing two pages if their associated probabilities (or probabilities over sets they support, given a list of pages already chosen) are equal in $\Gamma$, and no other engines support either page with positive probability.  
%
%As an example of the above issue, suppose there are two engines each with one slot, four pages, and the distribution over user types is uniform over those four pages (i.e.\ each user desires only a singleton).  Also suppose that $f_i(q_1, q_2) = q_i / (q_1 + q_2)$ (proportional choice).  In this case not all equilibria are pure: there is an equilibrium in which the first engine randomizes over pages $1$ and $2$, and the second engine randomizes over pages $3$ and $4$.  
%
%For ease of exposition, we will assume that page probabilities in $\Gamma$ are sufficiently distinct to avoid this possibility.  That is, given any choice $S$ of pages, and any two pages $p_1$ and $p_2$ not in $S$, we will assume that the probability that $p_1$ satisfies a user but $S$ does not is not equal to the probability that $p_2$ satisfies the user but $S$ does not.  We say that $\Gamma$ is \emph{non-degenerate} if this is true.  We note that our price of anarchy results will go through without this assumption, but making this assumption keeps our statements cleaner.

\begin{theorem}
\label{thm:beta0.pure}
Suppose that \TypeDist is in general position, and 
$\SelRule$ is non-indifferent.  
Then, every pure Nash Equilibrium of the game \SearchGame{0}{\TypeDist}
(that is, with $\DF=0$) is deterministic. 
\end{theorem}

\begin{proof}
Let $\mathcal{C}$ denote the support of \TypeDist.
Let $\MatchDists$ be a Nash Equilibrium of \SearchGame{0}{\TypeDist}.
(If no Nash Equilibrium exists, the claim holds vacuously.)
Because $\DF=0$, the utility of engine $i$ at this equilibrium is
\begin{align*}
\Payoff{i}{\MatchDists}
& = 
\sum_{S \subseteq \PageSet} \sum_{t \geq 0} 
\Td{S,t} \cdot \SelRule[i](\SatProbs(S,t,\MatchDists)) 
\cdot \SatProb{i}(S,t,\MatchDist{i}).
\end{align*}
Consider the deterministic strategy for player $i$ that selects the
permutation $\Matching$ with probability $1$.
The utility of this strategy is
\[ 
\sum_{S \subseteq \PageSet} \sum_{t \geq 0} 
\Td{S,t} \cdot \SelRule[i](1, \SatProbs_{-i}(S,t,\MatchDists_{-i})) 
\cdot \Indicator{\Matching([t]) \cap S \neq \emptyset}.
\] 
Because the strategy $\MatchDist{i}$ is utility-maximizing for engine
$i$, its utility is at least the utility of each pure strategy, and
hence at least the utility of any convex combination of pure strategies.
If we consider the convex combination in which each
permutation \Matching is assigned a weight of
$\MatchDist{i}(\Matching)$, this implies that
\begin{align}
\sum_{S \subseteq \PageSet} \sum_{t \geq 0} 
\Td{S,t} \cdot \SelRule[i](\SatProbs(S,t,\MatchDists))
\cdot \SatProb{i}(S,t,\MatchDist{i}) 
& \geq 
\sum_{S \subseteq \PageSet} \sum_{t \geq 0} 
\Td{S,t} \cdot \SelRule[i](1, \SatProbs_{-i}(S,t,\MatchDists)) 
\cdot \SatProb{i}(S,t,\MatchDist{i}).
\label{eq.pure.ineq}
\end{align}

Since $\SelRule[i](q_i, q_{-i})$ is non-decreasing in $q_i$, 
this inequality must be an equality.
And because $f$ is non-indifferent, this implies that for every
$(S,t) \in \mathcal{C}$ for which
$\SatProb{i}(S,t,\MatchDist{i}) > 0$, we must have either that
$\SatProb{i}(S,t,\MatchDist{i}) = 1$ or that
$\SatProb{j}(S,t,\MatchDist{j}) = 0$ for all $j \neq i$. 

Assume that $\MatchDist{i}$ is not a deterministic strategy.
Then there exist two non-equivalent permutations 
$\Matching, \Matching'$ with $\MatchDist{i}(\Matching) \in (0,1)$ and
$\MatchDist{i}(\Matching') \in (0,1)$.
Let $X \subseteq \mathcal{C}$ be the set of types 
satisfied by $\Matching$ but not by $\Matching'$,
and $X' \subseteq \mathcal{C}$ the set of types 
satisfied by $\Matching'$ but not by $\Matching$; 
note that $X \cup X' \neq \emptyset$ by non-equivalence.
We then have $\SatProb{i}(S,t,\MatchDist{i}) < 1$ 
for all $(S,t) \in X \cup X'$, and hence 
$\SatProb{j}(S,t,\MatchDist{j}) = 0$ for all $j \neq i$ and
$(S,t) \in X \cup X'$.
Thus, for each $(S,t), (S',t') \in X \cup X'$,
Equation~\eqref{eq.pure.ineq} implies that 
$\SelRule[i](\SatProbs(S,t,\MatchDists)) 
= \SelRule[i](1, \vc{0}) 
\; = \; \SelRule[i](\SatProbs(S',t',\MatchDists)).$
%\end{align*}
%\begin{align*} 
%\SelRule[i](\SatProbs(S,t,\MatchDists)) 
%& = \SelRule[i](1, \vc{0}) 
%\; = \; \SelRule[i](\SatProbs(S',t',\MatchDists)).
%\end{align*}

Because $\Gamma$ is in general position, 
$\sum_{(S,t) \in X} \Td{S,t} \neq \sum_{(S,t) \in X'} \Td{S,t}$;
w.l.o.g., assume that the left-hand side is larger.
Then, if engine $i$ were to increase the probability of the
permutation \Matching by some $\epsilon > 0$ while reducing the
probability of $\Matching'$ by $\epsilon$, 
the resulting change in utility would be 
\begin{multline*} 
\epsilon \cdot \Big( 
\sum_{(S,t) \in X} \Td{S,t} \SelRule[i](\SatProbs(S,t,\MatchDists)) 
- \sum_{(S,t) \in X'} \Td{S,t} \SelRule[i](\SatProbs(S,t,\MatchDists))
\Big) \\
 = \epsilon \cdot \SelRule[i](1, \vc{0}) \cdot
\Big( \sum_{(S,t) \in X} \Td{S,t} - \sum_{(S,t) \in X'} \Td{S,t} \Big)
\; > \; 0.
\end{multline*}
%
Engine $i$ could thus increase her utility by shifting
probability from \Matching to $\Matching'$,
contradicting the equilibrium assumption.
Thus \MatchDist{i} must be a deterministic strategy.
\end{proof}

\subsection{An Upper Bound on the Robust Price of Anarchy}
\label{sec:beta0-PoA-bound}

Theorem \ref{thm:beta0.pure} significantly simplifies the analysis of
our game
by letting us assume that all pure strategies are
deterministic. When the pure strategies are deterministic, the
resulting game is a monotone valid utility game (defined below), 
and monotone valid utility games are known to have robust Price of
Anarchy bounded by 2
\cite{vetta:nash,blum:hajiaghayi:ligett:roth,roughgarden:smoothness}.

More formally, we define a variant of the \SearchGameName, which we
call \DETGAME{\TypeDist}.  In this variant, search
engines are restricted to playing deterministic strategies ---
matchings between slots and pages.
We think of a matching as a set of pairs $(j,n)$, where $j$ is a slot
and $n$ a page.
As opposed to \SearchGame{0}{\TypeDist}, we allow
engines to play matchings that are not perfect, i.e., to leave some
pages out completely.

\begin{definition}[Valid Utility Game]
Consider a $k$-player game in which player $i$ has strategy space
$\Sigma_i = 2^{G_i}$ for some ground set $G_i$.
For a strategy profile $\vc{s} \in \Sigma_1 \times \Sigma_2 \times
\cdot \times \Sigma_k$, 
let $W(\vc{s})$ denote the welfare function of the
game, and $U_i(\vc{s})$ the utility of player $i$.
The game is a valid utility game if
(1) $W$ is a submodular function,
(2) $W(\vc{s}) \geq \sum_i U_i(\vc{s})$
for all strategy profiles $\vc{s}$, and 
(3) $U_i(\vc{s}) \geq W(\vc{s}) - W(\emptyset, \vc{s}_{-i})$
for each $i$ and strategy profile $\vc{s}$.
\end{definition}

\begin{lemma} \label{lem:deterministic-utility}
For every \TypeDist, \DETGAME{\TypeDist} is a valid utility game.
\end{lemma}

\begin{proof}
A pure strategy profile in \DETGAME{\TypeDist} is a vector
$\Matchings=(\Matching[1], \ldots, \Matching[\NUMENG])$ 
of matchings. 
Its welfare \Welfare{\Matchings} is simply defined by
Equation~\ref{eqn:searcher-utility} as for more general distributions
of permutations, and similarly for the engines' payoffs
\Payoff{i}{\Matchings}.

Write $u_i(\Matchings)$ for the utility of player $i$ when the engines select (deterministic) strategies $\Matchings$.  Define the total utility of the players given their matching choices, $u(\Matchings)$, to be the sum of the engines' utilities.  Note that $u(\Matchings)$ is precisely the probability that a user that arrives and selects an engine is ultimately satisfied. We also write $u(\Matching[i] | \Matchings_{-i})$ to be engine $i$'s marginal contribution to the overall utility, given the choices made by the other players.  That is, $u(\Matching[i] | \Matchings_{-i}) = u(\Matchings) - u( \emptyset, \Matchings_{-i})$ where $\emptyset$ is the strategy that leaves all slots empty.

To show that \DETGAME{\TypeDist} is a monotone valid-utility game, we verify
the following four properties:
%\begin{description}
%\item[\Welfare{\Matchings} is monotone]

\smallskip
\noindent
\emph{1. \Welfare{\Matchings} is monotone.}
Consider an engine $i$ adding a page $n$ to a slot $j$.
By monotonicity of the selection rule, this can only increase the
likelihood that a user who would be satisfied by page $n$ in slot $j$  
would visit engine $i$; because the strategy is deterministic, such a
user will be satisfied with probability 1 upon visiting engine $i$.
Thus, the probability that a user is ultimately satisfied cannot decrease.

%\item[\Welfare{\Matchings} is submodular]
\smallskip
\noindent
\emph{2. \Welfare{\Matchings} is submodular.}
Consider engine $i$ adding a page $n$ to slot $j$.
Let $\Matchings, \Matchings'$ be two strategy profiles
such that $\Matching[i]' \supseteq \Matching[i]$ for all $i$.
We will prove that the marginal increase from adding $n$ to
slot $j$ is no larger starting from $\Matchings'$ than from
\Matchings. 
We prove this individually for each user type $(S,t)$; the claim
follows by taking expectations over types.

Focus on a type $(S,t)$ from now on. If page $n$ in slot $j$ would not
satisfy the user, then the satisfaction probability stays the same;
therefore, so do the user's selection probabilities, and the increase
in welfare is 0 for both strategy profiles.
Otherwise, engine $i$ would now deterministically satisfy the user.
If the user would already be satisfied deterministically 
under $\Matching'$, then adding page $n$ does not change any
satisfaction probabilities, so the marginal increase in user welfare
is 0 from $\Matching'$, and it must be non-negative for $\Matching$ by
monotonicity.
This leaves the case when the user would not have been satisfied by
engine $i$ under $\Matching'$ (and thus also not under $\Matching$).
Then, the user's probability of visiting $i$ (and being satisfied) may
increase. Under $\Matching'$, the probability of being satisfied by
other engines $i' \neq i$ may also be 1 (when it was 0 in \Matching);
thus, by the monotonicity assumptions on selection rules, the
probability of visiting engine $i$ can only be smaller under
$\Matching' \cup \SET{(j,n)}$ than under $\Matching \cup \SET{(j,n)}$;
thus, the satisfaction probability can only increase by a smaller
amount, proving submodularity.

%\item[$\Welfare{\Matchings} \geq \sum_i \Payoff{i}{\Matchings}$]
\smallskip
\noindent
\emph{3. $\Welfare{\Matchings} \geq \sum_i \Payoff{i}{\Matchings}.$}
The utility of engine $i$ is the fraction of users it
satisfies. Summed over $i$, this is the total fraction of
users satisfied, which is the user welfare by definition.

%\item[$\Payoff{i}{\Matchings} \geq \Welfare{\Matchings} - \Welfare{\emptyset, \Matchings_{-i}}$]
\smallskip
\noindent
\emph{4. $\Payoff{i}{\Matchings} \geq \Welfare{\Matchings} - \Welfare{\emptyset, \Matchings_{-i}}.$}
The left-hand side is the fraction of users who visit engine $i$ and
are satisfied.
The right-hand side is the fraction of users who visit engine $i$ and
are satisfied, but would not have been satisfied had engine $i$ not
participated.
The former quantity is therefore at least as large as the latter. 
%\end{description}
\end{proof}

We can use Theorem~\ref{thm:beta0.pure} and
Lemma~\ref{lem:deterministic-utility} to obtain bounds on the Price of Anarchy.
%of
%the \SearchGameName.

\begin{theorem}
\label{thm:poa-beta0}
Let \TypeDist be in general position. 
Then, the Robust Price of Anarchy of the \SearchGameName with $\DF=0$
is at most $2$.
\end{theorem}

\begin{proof}
The welfare-optimal strategy profile \OPT for 
\SearchGame{0}{\TypeDist} is pure: randomization by the engines
can only increase the probability that a user will select an engine
that fails to satisfy him.
Thus, \OPT is also a valid strategy in \DETGAME{\TypeDist}, and
because the welfare functions coincide on permutations, it must also
be optimal.

Let \PermDists be any Nash Equilibrium strategy profile for
\SearchGame{0}{\TypeDist}. 
By Theorem~\ref{thm:beta0.pure}, the strategies in \PermDists must be
deterministic, i.e., individual permutations \Perm[i].
The strategies \Perm[i] are therefore also valid strategies
in \DETGAME{\TypeDist}. We claim that they also form an equilibrium in
that game.
First, because \PermDists is a Nash Equilibrium for
\SearchGame{0}{\TypeDist}, no player $i$ would prefer to deviate to
another permutation $\Perm[i]'$, i.e., no player prefers to deviate to
another complete matching. Deviating to an imperfect matching
\Matching[i] is always weakly dominated by deviating to a perfect
matching $\Matching[i]' \supseteq \Matching[i]$; but since $i$ does
not want to deviate to another permutation, no pure deviation is
beneficial. Finally, whenever a player $i$ can profitably deviate to a
distribution of strategies, she can also profitably deviate to at
least one of the strategies in the support of the distribution.
In summary, we have shown that $(\Perm[1], \ldots, \Perm[\NUMENG])$ is
an equilibrium of \DETGAME{\TypeDist}.
By Theorem~\ref{thm:roughgarden-robust-PoA}, the Robust Price of Anarchy of
monotone valid utility games is at most 2, so that the welfare of
$\PermDists$ is at least half the optimal welfare.
\end{proof}

%Note the following relationship between \DETGAME and the competitive search engine game.  For any strategy profile $\Matchings$ in \DETGAME, the corresponding (deterministic) strategy profile in the competitive search engine game results in the same utility profile for the sellers.  Let $\Matchings^*$ be a Nash equilibrium in \DETGAME.  Then, thinking of $\Matchings^*$ as a deterministic strategy profile in the original game, the equilibrium condition implies that no engine has a profitable deviation to a different deterministic strategy.  Moreover, Theorem \ref{thm:beta0.pure} implies that no engine has a utility-improving deviation to a non-deterministic strategy.  Thus $\Matchings^*$ is also a Nash equilibrium in the competitive search engine game.

The general bound of 2 for the robust Price of Anarchy of Valid
Utility Games was established by
Blum et al.~\cite{blum:hajiaghayi:ligett:roth} and 
Roughgarden~\cite{roughgarden:smoothness}, generalizing the theorem
of Vetta~\cite{vetta:nash} for the mixed Price of Anarchy.

\begin{theorem}[Roughgarden (Example~1.3 from \cite{roughgarden:smoothness})]
\label{thm:roughgarden-robust-PoA}
The robust Price of Anarchy of any valid utility game is at most 2.
\end{theorem}


\subsection{Alternative Proof -- Useful for Convexity}

\begin{theorem}
Let \TypeDist be in general position, and suppose that every correlated equilibrium of \SearchGameName has only deterministic strategies in its support.  Then the correlated price of anarchy of \SearchGameName is at most $2$.
\end{theorem}
\begin{proof}
Pick a threshold $t$, and consider the actions chosen at equilibrium given a particular signal.  By assumption these actions are deterministic, say matchings $\Matchings$.  Write $\Matchings'$ for the socially optimal matching profile.  For each $j$, write $\mu_j$ for the probability that a user is satisfied by profile $\Matchings[j]'$ but not by any $\Matching[i]$.  That is,
\[
\mu_j = \sum_{S \subseteq \PageSet} \sum_{t \geq 0} 
\Td{S,t} \cdot \Indicator{(\Matching[j]'([t]) \cap S \neq \emptyset) \wedge (\forall i \colon\ \Matching_i([t]) \cap S = \emptyset)}.
\]

Consider the utility of engine $i$ if he were to switch his action from $\Matching[i]$ to $\Matching[j]'$.  Under this new strategy profile, the engine would attract each user satisfied by $\Matchings[j]'$ but not any $\Matching[i]$.  The engine was potentially attracting some of these users already (and not satisfying them).  Moreover, the engine may lose some of the customers that he was satisfying when playing $\Matching[i]$.  Thus, the change in utility for engine $i$ is at least
\begin{align*}
& \mu_j  - \sum_{S \subseteq \PageSet} \sum_{t \geq 0} 
\Td{S,t} \cdot \SelRule[i](\SatProbs(S,t,\MatchDists)) 
\cdot \Indicator{(\Matching[j]'([t]) \cap S \neq \emptyset) \wedge (\forall i \colon\ \Matching_i([t]) \cap S = \emptyset)}\\
& \quad\quad - \sum_{S \subseteq \PageSet} \sum_{t \geq 0} 
\Td{S,t} \cdot \SelRule[i](\SatProbs(S,t,\MatchDists)) 
\cdot \Indicator{\Matching_i([t]) \cap S \neq \emptyset}.
\end{align*}

%\[ \mu_j - \Pr[ \text{user satisfied by $\Matching[j]'$ but not $\Matchings$ visits engine $i$ under $\Matchings$} ] - \Pr[ \text{user visits engine $i$ and is satisfied under $\Matchings$} ]. \]


By the equilibrium condition, this quantity must be non-positive.  Taking a sum over all $i$, we conclude
\begin{align*} 
& \sum_i \sum_{S \subseteq \PageSet} \sum_{t \geq 0} 
\Td{S,t} \cdot \SelRule[i](\SatProbs(S,t,\MatchDists)) 
\cdot \Indicator{\Matching_i([t]) \cap S \neq \emptyset} \\
& \quad + \sum_i \sum_{S \subseteq \PageSet} \sum_{t \geq 0} 
\Td{S,t} \cdot \SelRule[i](\SatProbs(S,t,\MatchDists)) 
\cdot \Indicator{(\Matching[j]'([t]) \cap S \neq \emptyset) \wedge (\forall i \colon\ \Matching_i([t]) \cap S = \emptyset)} \\
& \quad \geq \NUMENG \mu_j.
\end{align*}
Note that the first term on the LHS is precisely the social welfare of action profile $\Matchings$, and the second term is precisely $\mu_j$.  We therefore have that, for each $j$, $SW(\Matchings) \geq (\NUMENG-1) \mu_j$.  Taking a sum over all $j$, we conclude $\NUMENG SW(\Matchings) \geq (\NUMENG-1) \sum_j \mu_j$.  Note, however, that $\sum_j \mu_j$ is at most $OPT - SW(\Matchings)$, and thus we have 
\[ (2\NUMENG-1)SW(\Matchings) \geq (\NUMENG-1)OPT. \]
Since this holds for each signal in the correlated equilibrium, it holds in expectation over signals as well, and hence the price of anarchy is at most $2$ as required.

%Let $EQ_t$ be the multiset of pages chosen up to threshold $t$, and let $OPT_t$ be the socially optimal set of pages.  Let $EQ_t^i$ be the set of pages chosen by engine $i$ up to threshold $t$.  Write $k_p$ for the multiplicity of page $p$ in $EQ_t$; note $k_p$ is the number of sets $EQ_t^i$ in which $p$ appears.  Let $\phi$ be any mapping $\phi : OPT_t \to EQ_t$ such that $|\phi^{-1}(p)| = k_p$.  For each set of pages $S$, write $k_S$ for the number of engines that satisfy desire $S$ at the equilibrium corresponding to $EQ_t$.
%
%For each page $p \in OPT_t \backslash EQ_t$, write $v(p | EQ_t) = \sum_{S \ni p, S \cap EQ_t = \emptyset} \alpha_S$ for the probability that a user would be served by $p$ but not by any other page in $EQ_t$.  Note that, since the engine $i$ that chooses page $\phi(p)$ at equilibrium does not want to switch to page $p$, we must have that 
%\[ v(p | EQ_t) \leq \sum_{S: S \cap EQ_t^i = \{\phi(p)\} } \frac{\alpha_S}{k_S}. \]
%But now, writing $SW(OPT_t)$ and $SW(EQ_t)$ for the social welfare of the two page sets, respectively,
%\begin{align*}
%SW(OPT_t) - SW(EQ_t)
%& \leq \sum_{p \in OPT_t} v(p | EQ_t) \\
%& \leq \sum_{p \in OPT_t} \sum_{S: S \cap EQ_t^i = \{\phi(p)\}} \frac{\alpha_S}{k_S} \\
%& \leq \sum_{p' \in EQ_t} \sum_{i : p' \in EQ_t^i} \sum_{S : S \cap EQ_t^i = \{p'\} } \frac{\alpha_S}{k_S} \\
%& \leq \sum_{S : S \cap EQ_t \neq \emptyset} k_S \cdot \frac{\alpha_S}{k_S} \\
%& = SW(EQ_t)
%\end{align*}
%where the second-last inequality follows because the condition $S \cap EQ_t^i = \{p'\}$ implies that each set $S$ is counted at most once for each user that satisfies it.  Rearranging gives $SW(OPT_t) \leq 2SW(EQ_t)$.  Since our equilibrium constraints hold simultaneously for all thresholds, the result follows.
\end{proof}

%Given that search engines play pure strategies, we can demonstrate that the social welfare at equilibrium (i.e.\ the probability that a given agent is satisfied) is within a small constant of optimal.  

%This will require that $f$ have the following property: if $q_i$ is the only non-zero entry in $\mathbf{q}$, then $f_i(\mathbf{q}) = 1$.  Note: if instead we have $f_i(\mathbf{q}) \geq \gamma$ for some $\gamma$, then the price of anarchy degrades by a factor of at most $1/\gamma$.

\subsection{Necessity of Assumptions}
\label{sec:necessity}
At first sight, the assumptions of non-indifference of the \SelRule[i]
and general position of \TypeDist may appear like minor technical issues
that should be easily eliminated. 
However, we provide examples showing that, if either assumption is
removed, there are instances of the \SingletonGameName with
price of anarchy $\Omega(\NUMPAGES)$.  These examples appear
in Appendix \ref{app:necessity}.
%the bound in 
%Theorem~\ref{thm:poa-beta0} requires both assumptions, even for
%instances of the \SingletonGameName.

\bldelete{
\begin{example}[Necessity of Non-Indifference]
Consider an instance of the \SingletonGameName with \NUMPAGES pages
and $\NUMENG = \NUMPAGES+1$ engines. 
Choose any distribution \TypeDist in general position over these
singleton sets, subject to the constraint that 
$\Td{n} \in [\frac{2}{3\NUMPAGES}, \frac{4}{3\NUMPAGES}]$
for each page $n$.  

Consider the following selection rule.
First, engine $\NUMPAGES+1$ is selected with probability
$\SelRule[\NUMPAGES+1](\SatProbs) 
= 1 - \sum_{i \leq \NUMPAGES} \SelRule[i](\SatProbs)$, 
so it suffices to describe the selection rule on engines 
$i \leq \NUMPAGES$.
For each $i \leq \NUMPAGES$, if engine $i$ is the only engine in $[\NUMPAGES]$ 
with non-zero probability of displaying page $n$
(i.e., $q_i > 0$ and $q_j = 0$ for all $j \in [\NUMPAGES]\backslash\{i\}$),
then the user will always choose engine $i$, so $\SelRule[i](\SatProbs) = 1$.
Otherwise, let 
$\SelRule[i](\SatProbs) = \max(0, \min(\frac{1}{\NUMPAGES}, \half(1 - \sum_{j \in [\NUMPAGES]\backslash\{i\}} q_j)))$.
In other words, engine $i$ is selected with probability
$\half(1 - \sum_{j \in [\NUMPAGES]\backslash\{i\}} q_j)))$, but the value is
``truncated'' into the interval $[0,\frac{1}{\NUMPAGES}]$.  
Note that the \SelRule[i] are not non-indifferent, 
since $\SelRule[i](\SatProbs)$ does not depend on \SP{i}{n}
when $\SP{j}{n} \neq 0$ for any $j \in [\NUMPAGES]\backslash\{i\}$.
The selection rules \SelRule[i] are, however, non-decreasing in
\SP{i}{n} and non-increasing in \SP{j}{n} for $j \neq i$.

The socially optimal strategy profile is for each engine 
$i \leq \NUMPAGES$ to deterministically display page $i$. 
This profile leads to a welfare of $1$. 

We now describe an equilibrium profile.
Let $X = \big(\sum_{j  \in \PageSet} \frac{1}{\Td{j}} \big)^{-1}$.
Consider the symmetric profile in which every engine selects page $n$ with
probability $\rho_n = \frac{\Td{n}-X}{\Td{n}(\NUMPAGES-1)}$.
Note that since $\Td{n} \in [\frac{2}{3\NUMPAGES}, \frac{4}{3\NUMPAGES}]$ 
for each $n$, we have 
\begin{align*}
0 
& < \rho_n 
\; = \; \frac{1-\frac{X}{\Td{n}}}{\NUMPAGES-1} 
\; \leq \; \frac{1 - \frac{3\NUMPAGES/4}{3\NUMPAGES^2/2}}{\NUMPAGES-1}
\; \leq \; \frac{2}{\NUMPAGES}.
\end{align*}
Moreover, the values $(\rho_n)$ form a probability distribution (and
hence a valid strategy profile) since  
\begin{align*}
\sum_{n \in \PageSet} \rho_n 
& = \frac{1}{\NUMPAGES-1} \cdot \sum_j 
\left( 1 - \frac{1/\Td{j}}{\sum_{n \in \PageSet} 1/\Td{n}}\right) 
\; = \; \frac{1}{\NUMPAGES-1} \cdot
\left(\NUMPAGES - \frac{\sum_{j\in \PageSet} 1/\Td{j}}{\sum_{n \in \PageSet} 1/\Td{n}}\right)
\; = \; 1.
\end{align*}
Under this strategy profile, for engine $i \in [\NUMPAGES]$ and page
$n$, we have that
\begin{align*}
\SelRule[i](\SatProbs) 
& = \max\left(0, \min\left(\frac{1}{\NUMPAGES}, \half (1 - (\NUMPAGES - 1)\rho_n)\right)\right)
\; = \; \min\left(\frac{1}{\NUMPAGES}, \frac{X}{2\Td{n}}\right).
\end{align*}
Because $\Td{n'} \in [\frac{2}{3\NUMPAGES}, \frac{4}{3\NUMPAGES}]$ for
all pages $n'$, we get that $\Td{n} \leq 2X/\NUMPAGES$, which in turn
implies that $\frac{X}{2\Td{n}} \leq \frac{1}{\NUMPAGES}$,
so $\SelRule[i](\SatProbs) = \frac{X}{2\Td{n}}$.
The utility of engine $i \leq \NUMPAGES$ under this strategy profile
is therefore
\begin{align*}
\sum_n \Td{n} \SelRule[i](\SatProbs(n)) \cdot \SP{i}{n}
& = \sum_{n \in \PageSet} X/2 \cdot q_i(n) 
\; = \; X/2,
\end{align*}
which is independent of her strategy.
Thus, every strategy is a best-response for engine $i \leq \NUMPAGES$;
in particular, the proposed profile constitutes an equilibrium
for the engines $i \leq \NUMPAGES$.
Since the strategy of engine $\NUMPAGES+1$ does not influence the
payoff of the other engines, we may simply assume that engine
$\NUMPAGES+1$ plays some best response.

To bound the welfare of the equilibrium, we consider separately the
engines $i \leq \NUMPAGES$ and engine $\NUMPAGES+1$.
Engine $\NUMPAGES+1$ can satisfy a user with probability at most
$\max_n \SET{\Td{n}} = O(1/\NUMPAGES)$. 
For engines $i \leq \NUMPAGES$, because their strategies are
symmetric, the social welfare is precisely the probability that an
arbitrary engine satisfies a user type drawn from \TypeDist. 
This is at most 
$\NUMPAGES \cdot \max_n \SET{\rho_n} \cdot \max_n \SET{\Td{n}} =
O(1/\NUMPAGES)$.
The Price of Anarchy in this example is therefore $\Omega(\NUMPAGES)$. 
\end{example}

\begin{example}[Necessity of General Position]
Consider an instance of the \SingletonGameName with \NUMENG engines
and $\NUMPAGES = \NUMENG$ pages. 
The distribution over desired pages is uniform:
$\Td{n} = 1/\NUMPAGES$ for each page $n$.
The selection function is a weighted proportional rule: 
$\SelRule[i](\SatProbs) = \frac{w_i \SatProb{i}}{\sum_j w_j \SatProb{j}}$,
where $w_1 = \NUMENG^2$ and $w_j = 1$ for all $j \neq 1$. 
(In other words, users have a significant preference for engine 1.)

The socially optimal strategy profile is for each engine $i$ to
deterministically display page $i$ in her first slot; this leads to a
social welfare of $1$.
Consider the following strategy profile: 
engine $1$ selects one of pages $1$ through $\NUMENG-1$ uniformly at
random to display in her first slot, 
and all remaining engines deterministically display page \NUMENG in
their first slot with probability $1$.
We claim that this profile constitutes an equilibrium. 
To see why, note that engine $1$ does not compete with any other
engine for pages $1$ through $\NUMENG - 1$.
Thus, for any distribution $p$ over pages $1$ through $\NUMENG - 1$ 
chosen by engine $1$ for slot 1, her utility is 
$\sum_{n < \NUMENG} \frac{1}{\NUMENG} p(n) = \frac{1}{\NUMENG}$;
on the other hand, any weight placed on page \NUMENG is multiplied
by a factor strictly less than 1 due to the competition, 
and thus leads to a loss in utility.
On the other hand, if any other engine chooses to display in her first
slot a page $n < \NUMENG$, her utility conditioned on selecting that
page is $\frac{1}{\NUMENG} \cdot
\frac{1}{1+\NUMENG^2\frac{1}{\NUMENG-1}} < \frac{1}{\NUMENG^2}$,
which is the utility derived from page \NUMENG.
Thus, each engine $i > 1$ maximizes her payoff by displaying page
\NUMENG in her first slot with probability $1$.
In summary, this strategy profile is an equilibrium.

In this equilibrium, a user who desires page \NUMENG is satisfied
with probability $1$ (since he will choose any of the engines that
deterministically display it in the first slot), 
whereas any other user is satisfied with probability
$\frac{1}{\NUMENG-1}$ (since he must choose engine 
$1$, who displays the desired page with this probability).
The social welfare is thus 
$\frac{1}{\NUMENG} + \frac{\NUMENG-1}{\NUMENG}\cdot
\frac{1}{\NUMENG-1} = \frac{2}{\NUMENG}$;
hence, the Price of Anarchy in this example is $\Omega(\NUMENG)$. 
\end{example}
}

\ignore{%
\subsection{An Improved Analysis for Singleton Desired Sets}
The analysis can be improved slightly when searchers only desire
singleton sets; that is, $\SetCard{S} = 1$ for each $S$ in the support
of \TypeDist. (Notice that, contrary to the \SingletonGameName, we
still allow arbitrary threshold distributions.)
We prove a bound of $2-1/\NUMENG$ on the pure Price of Anarchy in this
case, and also provide an example demonstrating that this bound is
tight. Whether the analysis here can be extended to the robust Price
of Anarchy is an interesting open question.

\begin{theorem}
\label{thm:pure-singleton}
Let \TypeDist be in general position, and assume that
$|S| = 1$ for each $S$ in the support of \TypeDist.  
Also assume that the selection functions \SelRule[i] are
non-indifferent. 
Then, the pure Price of Anarchy of the \SearchGameName with $\DF=0$
is at most $2-1/\NUMENG$.
\end{theorem}

\dkcomment{At the moment, the proof seems to assume that the threshold
$t$ is fixed. It probably extends to thresholds being independent of
frequencies. The result might extend to general distributions, but
it's not completely obvious.}

\begin{proof}
Consider a pure-strategy equilibrium \EQ.
First, by Theorem~\ref{thm:beta0.pure}, \EQ must be deterministic,
i.e., each engine $i$ plays a deterministic pure strategy \Perm[i].
Write $\EQ[t] = \bigcup_i \PermS[i]{[t]}$ for the set of all pages
chosen by any engine within the first $t$ slots in \EQ, and let
$k_n$ be the number of engines that select page $n \in \EQ[t]$.
Let \OPT be an optimum solution, which is necessarily deterministic. 
Similar to \EQ[t], let \OPT[t] be the set of pages chosen in the
optimal solution by any engine, up to slot $t$.
Notice that the optimum solution avoids duplication, so for every $t$,
every page $n \in \OPT[t]$ is chosen by exactly one engine.

Suppose that a user has threshold $t$ and desired page $n$, drawn
jointly according to \TypeDist.
If there exists at least one engine with page $j$ within its first
$t$ slots, the user can choose one such engine and be satisfied with
probability $1$.  Thus the user will be unsatisfied if and only if $n$
does not appear within the first $t$ slots of any engine. 

\dkcomment{I edited up to here before abandoning it.}
Note that \OPT[t] is the set of pages that maximizes
$\sum_{p \in S} \alpha_p$, subject to each engine having at most
$t$ pages.  In particular, each page in $OPT_t$ is chosen by exactly
one engine.   

Note that, for every $p \in EQ_t$ and every $p' \in OPT_t \backslash EQ_t$, we have that $\frac{\alpha_p}{k_p} \geq \alpha_{p'}$  (since $EQ_t$ is an equilibrium).  This implies that $EQ_t \subseteq OPT_t$, ignoring multiplicities (since $OPT_t$ will contain exactly those pages with the highest values of $\alpha_p$).  

Since $EQ_t$ and $OPT_t$ have the same number of pages if we count multiplicities in $EQ_t$, there exists a mapping $\phi : OPT_t \to EQ_t$ such that $\phi(p) = p$ for all $p \in EQ_t$ and $|\phi^{-1}(p)| = k_p$ for each $p \in EQ_t$.

We now have
\begin{align*}
\sum_{p \in OPT_t} \alpha_p 
& = \sum_{p \in EQ_t} \alpha_p + \sum_{p' \in OPT_t \backslash EQ_t} \alpha_{p'} \\
& \leq \sum_{p \in EQ_t} \alpha_p + \sum_{p \in OPT_t \backslash EQ_t} \frac{\alpha_{\phi(p)}}{k_{\phi(p)}} \\
& = \sum_{p \in EQ_t} \alpha_p + \sum_{p \in EQ_t} \alpha_p \frac{k_p-1}{k_p} \\
& \leq (2-\frac{1}{\NUMENG}) \sum_{p \in EQ_t} \alpha_p
\end{align*}
where the equality on the second-last line is due to the fact that $|\phi^{-1}(p) \cap (OPT_t \backslash EQ_t)| = k_p - 1$ for all $p \in EQ_t$.
\end{proof}

We now show by way of an example that the bound of $2 - 1/\NUMENG$
from Theorem~\ref{thm:pure-singleton} is tight.

\begin{example}[Price of Anarchy exactly $2 - \frac{1}{\NUMENG}$]
The number of pages equals the number of engines, $\NUMPAGES = \NUMENG$. 
Each user has a threshold of $1$, 
and desires page $n$ with probability 
$\Td{(1,\SET{n})} = b_i / \sum_{n'} b_{n'}$, 
where $b_1 = n$ and $b_n = 1$ for all $n > 1$.
The selection rule is symmetric across engines.
In this case, an equilibrium is for all engines to display page $1$ in
their first slot deterministically.
(Each engine has utility $1/\NUMENG$, and would achieve strictly lower
utility by deviating to another page.)
This equilibrium has social welfare of $(2-1/\NUMENG)^{-1}$.  
The socially optimal solution has each engine $i$ deterministically
displaying page $i$ in her first slot, for a social welfare of $1$.
The Price of Anarchy is therefore at least $(2-1/\NUMENG)$.
\end{example}
}

%\blcomment{While I agree that it should be possible to prove this
%  robustly, it turns out that the game is only $(1, 1)$-smooth, which
%  implies a PoA of 2.  Consider an instance with $3$ pages and $3$
%  engines.  The selection rule is majority selection, with ties broken
%  as $f_1(1,1,0) = 1$, $f_2(0,1,1) = 1$, $f_3(1,0,1) = 1$.  Let $s$ be
%  the strategy where engine $i$ chooses page $i$.  Let $s'$ be the
%  strategy where engine $1$ chooses page $3$, $2$ chooses $1$, and $3$
%  chooses page $2$.  Then $SW(s) = 1$, $SW(s') = 1$, but $u_1(s_1',
%  s_2, s_3) = 0 = u_2(s_1, s_2', s_3) = u_3(s_1, s_2, s_3')$.  So in
%  this case the game is $(1,1)$-smooth, which gives a price of anarchy
%  of $2$.}

%\subsection{Non-existence of Pure Equilibria}
%\label{sec:non-existence}
%We justify the broadened focus on the robust Price of Anarchy by
%showing here that even the \SingletonGameName with $\DF=0$ may not
%have any pure Nash Equilibria.
%We construct an instance with $\NUMPAGES=2$ pages and $\NUMENG=3$
%engines. The page request probabilities are in general position,
%with $\Td{n} \in (\third, \frac{2}{3})$ for $n=1,2$.  
%The selection rule is as follows.
%For given $\SatProbs$, define 
%$\gamma_i = \SatProb{i} \cdot 2^{(\SatProb{i+1} - \SatProb{i+2})}$, 
%with indices taken mod $3$. 
%The selection rule is then 
%$\SelRule[i](\SatProbs) = \gamma_i/(\gamma_1 + \gamma_2 + \gamma_3)$.  
%For example, $\SelRule[1](1,1,0) = 4/5$, 
%whereas $\SelRule[1](1,0,1) = 1/5$.
%Note that the \SelRule[i] satisfy the non-indifference property. 
%
%By Theorem~\ref{thm:beta0.pure}, if a pure equilibrium exists, it must
%be a profile of deterministic strategies.  There are two cases.  
%First, if all three engines select the same page $n$, then the
%utility of each engine is 
%$\Td{n} \cdot \SelRule[i](1,1,1) = \Td{n} \cdot \third < 2/9$.
%In this case, each engine would benefit by switching to the other
%page, which would give a utility of $\third > 2/9$. 
%Thus, this profile cannot be an equilibrium.
%
%The second case is that two engines select one page, and the third
%engine selects the other.
%By symmetry, we can assume that engines $1$ and $2$ select the same
%page $n$.  In this case, the utility of engine $2$ is 
%$\Td{n} \cdot \SelRule[2](1,1,0) = \Td{n} \cdot \frac{1}{5} \leq 2/15$.
%Note, then, that engine $2$ would benefit by switching to the other
%page $n'$; her utility would become 
%$\Td{n'} \cdot \SelRule[2](0,1,1) = \Td{n'} \cdot \frac{4}{5} > 4/15$.
%This profile is therefore not an equilibrium, either.
%As we have exhausted all possibilities for a pure equilibrium, 
%we conclude that no pure equilibrium exists.

%\paragraph{Price of anarchy for non-singleton desires.}
%
%If a user can desire multiple pages, we can still bound the price of anarchy.  
%%Currently the best bound I can come up with is $2$, though I believe that the correct bound is still $2-1/n$.  Here is a proof of $2$.  TODO: improve this to $2 - 1/n$.
%
%BRENDAN:  Todo -- prove this using valid utility games.  Also, do this before the $2 - 1/n$ bound.
%
%\begin{theorem}
%Suppose $\beta = 0$, $f$ is non-indifferent, and $\Gamma$ is non-degenerate.  Then the price of anarchy of the search engine game is at most $2$.
%\end{theorem}
%\begin{proof}
%Pick a threshold $t$.  Let $EQ_t$ be the multiset of pages chosen at equilibrium up to threshold $t$, and let $OPT_t$ be the socially optimal set of pages.  Let $EQ_t^i$ be the set of pages chosen by engine $i$ up to threshold $t$ at equilibrium.  Write $k_p$ for the multiplicity of page $p$ in $EQ_t$; note $k_p$ is the number of sets $EQ_t^i$ in which $p$ appears.  Let $\phi$ be any mapping $\phi : OPT_t \to EQ_t$ such that $|\phi^{-1}(p)| = k_p$.  For each set of pages $S$, write $k_S$ for the number of engines that satisfy desire $S$ at the equilibrium corresponding to $EQ_t$.
%
%For each page $p \in OPT_t \backslash EQ_t$, write $v(p | EQ_t) = \sum_{S \ni p, S \cap EQ_t = \emptyset} \alpha_S$ for the probability that a user would be served by $p$ but not by any other page in $EQ_t$.  Note that, since the engine $i$ that chooses page $\phi(p)$ at equilibrium does not want to switch to page $p$, we must have that 
%\[ v(p | EQ_t) \leq \sum_{S: S \cap EQ_t^i = \{\phi(p)\} } \frac{\alpha_S}{k_S}. \]
%But now, writing $SW(OPT_t)$ and $SW(EQ_t)$ for the social welfare of the two page sets, respectively,
%\begin{align*}
%SW(OPT_t) - SW(EQ_t)
%& \leq \sum_{p \in OPT_t} v(p | EQ_t) \\
%& \leq \sum_{p \in OPT_t} \sum_{S: S \cap EQ_t^i = \{\phi(p)\}} \frac{\alpha_S}{k_S} \\
%& \leq \sum_{p' \in EQ_t} \sum_{i : p' \in EQ_t^i} \sum_{S : S \cap EQ_t^i = \{p'\} } \frac{\alpha_S}{k_S} \\
%& \leq \sum_{S : S \cap EQ_t \neq \emptyset} k_S \cdot \frac{\alpha_S}{k_S} \\
%& = SW(EQ_t)
%\end{align*}
%where the second-last inequality follows because the condition $S \cap EQ_t^i = \{p'\}$ implies that each set $S$ is counted at most once for each user that satisfies it.  Rearranging gives $SW(OPT_t) \leq 2SW(EQ_t)$.  Since our equilibrium constraints hold simultaneously for all thresholds, the result follows.
%\end{proof}
%
%\paragraph{Removing the non-degeneracy assumption}
%
%If we remove the non-degeneracy assumption on $\Gamma$, then there may exist mixed equilibria.  However, in any such equilibrium, an engine mixes only over pages for which it is the only supporting engine.  This should not degrade social welfare: users of the given types will all choose the relevant engine with probability $1$, so this mixed equilibrium simply distributes the probability that a user is satisfied between multiple types, rather than concentrating this probability on a particular user type.  The price of anarchy should thus still be $2 - 1/n$, I think.  TODO: prove this.



